VenoMave: Targeted Poisoning Against Speech Recognition

Despite remarkable improvements, automatic speech recognition is susceptible to adversarial perturbations. Compared to standard machine learning architectures, these attacks are significantly more challenging, especially since the inputs to a speech recognition system are time series that contain both acoustic and linguistic properties of speech. Extracting all recognition-relevant information requires more complex pipelines and an ensemble of specialized components. Consequently, an attacker needs to consider the entire pipeline. In this paper, we present VENOMAVE, the first training-time poisoning attack against speech recognition. Similar to the predominantly studied evasion attacks, we pursue the same goal: leading the system to an incorrect and attacker-chosen transcription of a target audio waveform. In contrast to evasion attacks, however, we assume that the attacker can only manipulate a small part of the training data without altering the target audio waveform at runtime. We evaluate our attack on two datasets: TIDIGITS and Speech Commands. When poisoning less than 0.17% of the dataset, VENOMAVE achieves attack success rates of more than 80.0%, without access to the victim's network architecture or hyperparameters. In a more realistic scenario, when the target audio waveform is played over the air in different rooms, VENOMAVE maintains a success rate of up to 73.3%. Finally, VENOMAVE achieves an attack transferability rate of 36.4% between two different model architectures.

==> sections/algsimple.tex <==
\definecolor{commentcolor}{HTML}{2F538F}
\newcommand\mycomment[1]{{\Comment{\footnotesize\textcolor{commentcolor}{#1}}}}

\begin{algorithm}
\caption{\sys{}}
\label{alg:method}
\textbf{Input:} \\
\hspace*{\algorithmicindent} \(\inputaudio_t\) \mycomment{Target audio waveform} \\
\hspace*{\algorithmicindent} $\word$ \mycomment{Adversarial word sequence} \\
\hspace*{\algorithmicindent} $\trainset$ \mycomment{The training dataset} \\
\hspace*{\algorithmicindent} $\surrogatehmm$ \mycomment{Surrogate \ac{HMM}} \\

\begin{algorithmic}[1]
    \State \(\advpairsset\) \(\gets\) get\_adv\_states\_pairs($\inputaudio$, $\word$) \mycomment{Select the $\numadvpair$ pairs of frames that needs to be changed}
    \State $[\poisonframe]^\numadvpair$ \(\gets\) select\_poisons(\(\advpairsset\)) \mycomment{For each pair of <\originalstate, \adversarialstate>, we select $\numpois_\originalstate$ poison frames~$\poisonframe$}
    
    \For{$\indexone=1$ {\bfseries to} $\maxiter$}
    
    \For{$\modelindex=1$ {\bfseries to} \(\nummodels\)}
        \State $\model^{(\modelindex)}$ \(\gets\) train\_model($\trainset$)
    \EndFor
    
    \For{$\indextwo=1$ {\bfseries to} $\maxiterbulleye$}
        \State $\loss^{(\indextwo)}$ \(\gets\) 0 \mycomment{Set loss to zero}
        \For{$\poisonframe^\poisonindex$ {\bfseries in} $[\poisonframe]^\numadvpair$}
        \State $\loss^{(\indextwo)}$ \(\gets\) $\loss^{(\indextwo)}$ + Eq1\_loss($\poisonframe^\poisonindex$, $\originalframe^\poisonindex$, $\targetframe$, $[\model]^M$) \mycomment{Equation~\eqref{eq:BPLoss}}
        \EndFor
        \State $\loss^{(\indextwo)}$ \(\gets\) \(\frac{\loss^{(\indextwo)}}{\textrm{len}([\poisonframe]^\numadvpair)}\) \mycomment{Average of the loss}
        \State $[\poisonframe]^\numadvpair$ \(\gets\) update($[\poisonframe]^\numadvpair$, $\nabla \loss^{(\indextwo)}$) \mycomment{update all poison frames~\([\poisonframe]^\numadvpair\) using \(\nabla \loss^{(\indextwo)}\)}
    \State \textbf{break} if $\loss^{(\indextwo-1)} - \loss^{(\indextwo)} $ < 0.0001
    \EndFor
    
    \State $\trainset$ \(\gets\) updated($\trainset$, $[\poisonframe]^\numadvpair$) \mycomment{update $\trainset$ with new poisons $[\poisonframe]^\numadvpair$}
        
    \State $\victimmodel$ \(\gets\) train\_model($\trainset$) 
    \State $\hat{\word}$ \(\gets\) eval\_victim($\surrogatehmm$, $\inputaudio_t$, $\surrogatehmm$) \mycomment{get word sequence recognized by $\victimmodel$}
    \State \textbf{break} if $\hat{\word} = \word $
    
    \EndFor

\end{algorithmic}
\end{algorithm}


==> sections/background_old.tex <==
In this work, we propose \sys{}, the first targeted data poisoning attack against \ac{ASR} systems. % which employs a neural network along with an \ac{HMM}.
% While crafting poison audio waveforms, we practice \psycho{} modeling to introduce less perceptible noise. 
The following section provides the fundamental concepts of \ac{ASR} systems and \psycho{}~modeling that is used to reduce the amount of perceptible noise. % as far as it is necessary to understand our approach.
\subsection{Speech Recognition Systems}
In contrast to an end-to-end system, a hybrid \ac{ASR} system combines two models, a \ac{DNN} for acoustic modeling and the a \ac{HMM} that is used as language model for cross-temporal information integration, after the input has been initially processed by the~\ac{DNN}.
%
Hybrid systems still represent the state-of-the-art approach in \ac{ASR}, given that they are not as data-hungry as end-to-end systems~\cite{Andrusenko2020}. Furthermore, their architecture allows the user to explicitly specify task grammars and adapt language models on the fly. Additionally, hybrid \ac{ASR} systems still provide the best results in practice and typical benchmark tasks~\cite{du-16-chime-4, kanda-18-chime-5, medennikov-18-chime-5}. 
Such advantages have made them very popular for many commercial systems such as Amazon's Alexa and the system of choice for pre-trained embedded models that may not have the luxury of a big-data backend for adaptation~\cite{schoenherr-20-unacceptable}. %In the research area,
%Kaldi~\cite{povey2011kaldi} is one of the most popular tools that follows this approach, which also forms the basis of a number of commercial systems.

Figure~\ref{fig:asr_overview} provides an overview of the main system components:
\label{sec:prepro}

\begin{figure*}
    \centering
    \includegraphics[width=2.1\columnwidth]{figures/asr_overview/speech-poisoning-ASR.pdf}
    \caption{Overview of a state-of-the-art hybrid ASR system with two main components: the neural network calculates pseudo-posteriors of HMM states, and the decoder employs an HMM to generate the transcription.}
    \label{fig:asr_overview}
\end{figure*}

% \begin{figure*}
%     \centering
%   \includegraphics[width=1.8\columnwidth]{figures/asr_overview/asr_overview.pdf}
%     \caption{\TODO{replace figure (copied from another paper)}Overview of a state-of-the-art hybrid ASR system with the three main components of the ASR system: feature extraction, calculating pseudo-posteriors with a DNN, and decoding.}
%     \label{fig:asr_overview}
% \end{figure*}

\begin{itemize}%[itemsep=0pt, partopsep=4pt, parsep=4pt]
\item[(i)]\textbf{Feature Extraction.}
The raw waveform input is typically processed into a feature representation that should ideally preserve all relevant information (\eg phonetic information that describes the smallest acoustic unit of speech) while discarding the unnecessary remainders (\eg acoustic properties of the room).
We divide the input waveform into overlapping frames of fixed length, and process each frame using the \ac{DFT} to obtain a frequency representation in form of a spectrogram. 
We further calculate \acp{MFCC} features~\cite{stevens-37-scale} that consider the logarithmic frequency perception of the human auditory system and which are commonly used for speech. For this purpose, a Mel-scaled filterbank~\cite{shannon-03-comparative} is applied to the spectrogram representation and the output further processed by applying a \ac{DCT}. The resulting \ac{MFCC} features are augmented by their first and second derivatives to represent the temporal structure of the input. % data by \ac{ASR} systems as the input for the \ac{DNN}.
% We further calculate the logarithm of the magnitude spectrum  and apply a Mel filter bank to the resulting signal. The Mel filter bank is a psychoacoustic filter bank that scales the magnitude spectrum based on human listeners judgment of frequency perception~\cite{stevens-37-scale}.
% Then, a \ac{DCT} is applied and the resulting features are generally augmented via their first and second derivation. 
% These features, so-called \acp{MFCC}, are a very common feature representation for \ac{ASR} systems. These features are used as input for the neural network. % , a frame is additionally augmented by context frames to include time-depended information 

\item[(ii)]\textbf{Neural Network.}
In hybrid \ac{ASR} systems, \acp{DNN} are typically used as an acoustic model to describe the probabilities of \ac{HMM} states.
The \ac{HMM} mainly describes the language grammar, a phonetic-based word description of all words, and context-dependencies of phonetic units and words.
% The \ac{DNN} generates pseudo-posteriors, which are used during decoding. % to find the most likely word sequence.

 \item[(iii)]\textbf{Decoding.}
The decoding in hybrid \ac{ASR} systems utilizes some form of graph search on top of the neural network's output to infer the most probable word sequence from the acoustic signal.
%
For this purpose, the \ac{HMM} is used to find an optimal path (which is interpreted as a sequence of words) through the \ac{HMM} via Viterbi decoding~\cite{omura-69-viterbi}.

\end{itemize}  

\mypar{Viterbi training.}
During training of an \ac{ASR} system, the exact alignment between utterances and transcriptions and therefore the labels are typically unknown. To account for this, \emph{Viterbi training} is commonly utilized.

Starting with a training on equally aligned labels an initial neural network is trained, followed by a decoding of the training data. The resulting alignment is further used as the new alignment for the labels. 
% Typically, the neural network is initially trained on equally aligned labels. Then, the decoding is performed on the training data, and the resulting alignment is used as a new alignment for the labels. 


\subsection{\Psycho{} Modeling}
\label{sec:bg:psycho-modeling}
Recent adversarial examples against \ac{ASR} systems~\cite{schonherr2018adversarial, qin2019imperceptible} practiced \psycho{} hiding to introduce less perceptible adversarial noise.
Similar to Sch\" oenherr~\etal~\cite{schonherr2018adversarial}, we enforce \psycho{} modeling in some experiments to assess its affects on \sys{}.

\Psycho{} hearing thresholds generally describe how the dependencies between certain frequencies can lead to masking effects in the human perception.
The most common application of \psycho{} modeling is high-quality lossy signal compression, \eg{} MP3 compression~\cite{iso-93-part3}.
By utilizing a set of empirical hearing thresholds, the \psycho{} model of MP3 compression removes parts of a given digital audio signal that are inaudible.
Thus, the original input signal will be transformed into a smaller but lossy representation.

\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/psycho_freq_mask.pdf}
    \caption{Human hearing thresholds in quiet (solid blue line) versus a X dB masking tone at XX kHz (dashed line). The dashed line illustrates how a loud tone at XX kHz increases the hearing thresholds of nearby frequencies.}
    \label{fig:psycho_modeling}
\end{figure}

Figure~\ref{fig:psycho_modeling} shows a simple example of masking effects.
The solid blue line represents the human hearing thresholds in \emph{quiet} over the human-perceptible frequency range (i.e., 20 Hz to 20 kHz).
This is known as the \emph{absolute hearing thresholds}; the necessary sound pressures for each frequency to be audible in a \emph{quiet} environment.
Everything below this line is imperceptible in principle by humans.
However, this area gets bigger in the presence of another sound— a so-called masking tone, which changes the described hearing thresholds based on its sound pressure and frequency.
Figure~\ref{fig:psycho_modeling} also shows an example of a 1 kHz masking tone, where the dashed line reflects the decrease in sensitivity in the frequencies around the masking tone.



==> tables/boundedperturbation.tex <==
\begin{table*}[th]
\caption{Evaluation of \sys{} under perturbation bounds. For this experiment, we focus on four examples with which \sys{} has succeeded in fooling the victim (\(\poisonbudget=0.04\)).}
\centering
\smallskip
\normalsize
%\resizebox{.8\columnwidth}{!}{
\begin{tabular}{l|c c c | r r | c r r} 
\toprule
\multicolumn{1}{c}{\textbf{Perturbation}} & \multirow{2}{*}{\textbf{Speaker}} & \textbf{Original} & \textbf{Target} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SNRseg}}} & \multicolumn{1}{c}{\textbf{Maximum}} & \multicolumn{1}{c}{\textbf{Attack}} & \multicolumn{1}{c}{\textbf{Attack}} & \multicolumn{1}{c}{\textbf{Clean test}}\\
\multicolumn{1}{c}{\textbf{cap}} &  & \textbf{digit} & \textbf{digit} &  & \multicolumn{1}{c}{\textbf{perturbation \(\maxdelta\)}} & \multicolumn{1}{c}{\textbf{successful?}} & \multicolumn{1}{c}{\textbf{accuracy}} & \multicolumn{1}{c}{\textbf{accuracy}}\\
\midrule
Not bounded & IA & 7 & 2 &          3.38 & 0.098    & \cmark & 5.00     & 97.52 \\
Not bounded & IB & 2 & 4 &          6.35 & 0.092    & \cmark & 0.00     & 97.67 \\
Not bounded & IP & 3 & 6 &          -6.27 & 0.236   & \cmark & 13.33    & 97.94 \\
Not bounded & HJ & 7 & Z &          3.98 & 0.199    & \cmark & 5.56     & 97.38 \\
\midrule
0.080       & IA & 7 & 2 &          2.62 & 0.080    & \cmark & 25.00    & 97.56 \\
0.080       & IB & 2 & 4 &          5.91 & 0.080    & \cmark & 0.00     & 97.64 \\
0.080       & IP & 3 & 6 &          -9.68 & 0.080    & \cmark & 13.33    & 97.96     \\
0.080       & HJ & 7 & Z &          7.26 & 0.080    & \cmark & 5.56     & 97.31 \\
% \textbf{\netTwoLayer{}}	        & Two hidden layers, each with 100 neurons      & 54,895    & 98.75 	\\
% \textbf{\netTwoLayerPlus{}} 	& Two hidden layers, with 100 and 200 neurons	& 100,095   & 98.79	    \\
% \textbf{\netThreeLayer{}} 		& Three hidden layers, each with 100 neurons 	& 64,995    & 98.41	    \\

\bottomrule
\end{tabular}
%}
\label{table:exp:boundedperturbation}
\end{table*}

==> tables/diff_victim_settings.tex <==
\begin{table*}[t]
\addtolength{\tabcolsep}{-2pt}
\caption{Limited-knowledge adversary. 
% The poison budget~\(\poisonbudget\) is set to 0.005, while \psycho{} filtering is disabled.
For comparison, the first row represents the full-knowledge threat model. The next three rows represent when the victim uses a different network architecture, \netTwoLayer{}, \netThreeLayer{}, and \netThreeLayerPlus{}, respectively. Rows 5-8 show the attack statistics for when the adversary does not know the training parameters and the neural network architecture.}
\label{table:diffVictimSettings}
\begin{tabular}{l|ccccc|cc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Attacker settings}}} & \multicolumn{5}{c|}{\textbf{Victim settings}} & \multicolumn{1}{c|}{\textbf{Attack succ.}} & \multicolumn{1}{c}{\textbf{Clean test}} \\
 & \multicolumn{1}{c}{\textbf{Network}} & \multicolumn{1}{l}{\textbf{Learning rate}} & \multicolumn{1}{l}{\textbf{Dropout}} & \multicolumn{1}{l}{\textbf{Batch size}} & \multicolumn{1}{c|}{\textbf{Epochs}} & \multicolumn{1}{c|}{\textbf{rate (\%)}} & \multicolumn{1}{c}{\textbf{acc. (\%)}} \\
\midrule
\multirow{9}{*}{{\shortstack[l]{Network=\netTwoLayerPlus{}, \\batch size=32, \\dropout=0.2, \\learning rate=1e-4, \\DNN training epochs=25N}}} & \netTwoLayerPlus{} & 1e-4 & - & 32 & 15N+3V+15N & \multicolumn{1}{c|}{86.67} & 97.84 \\ \cmidrule{2-8} 
 & \netTwoLayer{} & 1e-4 & - & 32 & 15N+3V+15N & \multicolumn{1}{c|}{80.00} & 97.49 \\
 & \netThreeLayer{} & 1e-4 & - & 32 & 15N+3V+15N & \multicolumn{1}{c|}{83.33} & 97.55 \\
  & \netThreeLayerPlus{} & 1e-4 & - & 32 & 15N+3V+15N & \multicolumn{1}{c|}{X} & Y \\
 \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
 & \netTwoLayerPlus{} & 4e-4 & 0.2 & 64 & 10N+2V+20N & \multicolumn{1}{c|}{83.33} & 97.94 \\ \cmidrule{2-8} 
 & \netTwoLayer{} & 4e-4 & 0.2 & 64 & 10N+2V+20N & \multicolumn{1}{c|}{86.67} & 97.92 \\
 & \netThreeLayer{} & 4e-4 & 0.2 & 64 & 10N+2V+20N & \multicolumn{1}{c|}{86.67} & 98.04\\ 
 & \netThreeLayerPlus{} & 4e-4 & 0.2 & 64 & 10N+2V+20N & \multicolumn{1}{c|}{X} & Y\\ 
 \bottomrule
\end{tabular}
\vspace{-1em}
\end{table*}

% \addtolength{\tabcolsep}{-3pt}


==> tables/dropout.tex <==
\begin{table}[t]
\vspace{-0.2cm}
\caption{Evaluation of \sys{} when the victim employs dropout probability of 0.2. \netTwoLayerPlus{} is used  with \(\poisonbudget=0.04\).
%Note that the process of selecting the candidate frames to be poisoned does not depend on whether dropout is being used or not.
}
\centering
\smallskip
\scriptsize
%\resizebox{.8\columnwidth}{!}{
\begin{tabular}{l|r r} 
\toprule
 & \multicolumn{2}{c}{\textbf{Dropout}} \\ \cmidrule[0.6pt]{2-3}
 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{\textbf{0.2}} \\
\midrule
\textbf{Poisoned frames SNRseg}                 & 4.56          & 3.71              \\
\textbf{Maximum perturbation}                   & 0.151         & 0.148             \\
\textbf{Poisoned data length (in seconds)}      & 128           & 143               \\
\textbf{\# Poisoned data samples}               & 1,204         & 1,198             \\
\midrule
\textbf{Attack success rate (\%)}	            & 73.33         & 66.67             \\
\midrule
\textbf{Clean test accuracy (\%)} 		        & 97.86         & 97.98             \\

\bottomrule
\end{tabular}
%}
\label{table:exp:dropout}
\vspace{-0.3cm}
\end{table}



==> tables/exp_diffnets.tex <==
\begin{table}[t]
\vspace{-0.5cm}
\caption{Evaluation of \sys{} when the victim employs three different neural networks. Note that \(\poisonbudget\) is set to 0.04.}
\centering
\smallskip
\normalsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|r r r} 
\toprule
 & \multicolumn{3}{c}{\textbf{Victim's network}} \\ \cmidrule[0.6pt]{2-4}
 & \multicolumn{1}{c}{\textbf{\netTwoLayerPlusBold{}}} & \multicolumn{1}{c}{\netThreeLayerBold{}} & \multicolumn{1}{c}{\netTwoLayerBold{}} \\
\midrule
\textbf{Poison frames SNRseg}                   & 4.56          & 4.86          & 4.31          \\
\textbf{Maximum perturbation~$\maxdelta$}       & 0.151         & 0.167         & 0.175         \\
\textbf{Poisoned data length (in seconds)}      & 128           & 187           & 163           \\
\textbf{\# Poisoned data samples}               & 1,204         & 1,416         & 1,195         \\
\midrule
\textbf{Attack success rate (\%)}	            & 73.33         & 73.33         & 86.67         \\
\midrule
\textbf{Clean test accuracy (\%)} 		        & 97.86         & 97.34         & 97.48         \\

\bottomrule
\end{tabular}
}
\label{table:exp:diffnets}
\vspace{-0.3cm}
\end{table}



==> tables/individualspeaker.tex <==
\begin{table}[th]
\caption{Attack generalization accuracy of \sys{} per individual example. Those examples that we have not observed any generalization across all experiments are excluded from the table. It should be noted that we perform the \sys{} attack for 12 different examples in total.}
\centering
\smallskip
\normalsize
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c  r r} 
\toprule
\multirow{2}{*}{\textbf{Speaker ID}} & \multicolumn{1}{c}{\textbf{Original}} & \multicolumn{1}{c}{\textbf{Target}} &  \multicolumn{2}{c}{\textbf{Attack generalization}} \\
 & \multicolumn{1}{c}{\textbf{digit}} & \multicolumn{1}{c}{\textbf{digit}} &  \multicolumn{2}{c}{\textbf{accuracy (\%)}} \\ \cmidrule[0.6pt]{4-5}
 & & & \netTwoLayerPlusBold{} & \netThreeLayerBold{} \\
\midrule
HR              &       9   &   1      & 70.59      & 58.82      \\
IA              &       9   &   2      & 31.58      & 42.11      \\
IB              &       Z   &   4      & ~6.25       & 12.50       \\
IA              &       7   &   2      & 15.00         & 40.00         \\
IA              &       7   &   2      & 00.00          & 33.33      \\
\bottomrule
\end{tabular}
}
\label{table:exp:diffpoisonbudget:individualspeakers}
\end{table}

==> tables/results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \centering
% \smallskip
% \scriptsize
\begin{table*}[]
\centering
\smallskip
% \scriptsize
\caption{Evaluation of \sys{} when different levels of poison budget~\(\poisonbudget\) and \psycho{} filtering~\(\hearingOffset\) are used. When \(\poisonbudget\) is fixed, the same poison samples and frames are used regardless of \(\hearingOffset\). In this experiment, the victim \ac{ASR} system is built from scratch with the same settings that were used to build the surrogate networks, however, with a different random seed.}
\begin{tabular}{c||r|r||c||r|r||r|r}
\multirow{2}{*}{\textbf{\(\mathbf{\poisonbudget}\)}} & \multicolumn{2}{c||}{\textbf{Poisoned data}} & \multirow{2}{*}{\textbf{\(\bm{\hearingOffset}\)}} & \multicolumn{1}{c|}{\textbf{Poisoned frames}} & \multicolumn{1}{c||}{\textbf{Max perturbation}} & \multicolumn{1}{c|}{\textbf{Attack success}} & \multicolumn{1}{c}{\textbf{Clean test}} \\
 & \multicolumn{1}{c|}{\textbf{length (seconds)}} & \multicolumn{1}{c||}{\textbf{samples}} &  & \multicolumn{1}{c|}{\textbf{SNRseg}} & \multicolumn{1}{c||}{\textbf{\(\maxdelta\)}} & \multicolumn{1}{c|}{\textbf{rate (\%)}} & \multicolumn{1}{c}{\textbf{acc. (\%)}} \\
 \toprule
 \multirow{6}{*}{0.01} & \multirow{6}{*}{48.73} & \multirow{6}{*}{693.57} & 10 & 7.59 & 0.15 & 0.00 & 97.76 \\
 &  &  & 20 & 5.32 & 0.21 & 10.00 & 97.70 \\
 &  &  & 30 & 5.09 & 0.20 & 60.00 & 97.74 \\
 &  &  & 40 & 4.91 & 0.16 & 73.33 & 97.73 \\
 &  &  & 50 & 4.98 & 0.15 & 90.00 & 97.76 \\
 &  &  & \texttt{NONE} & 3.76 & 0.16 & 83.33 & 97.76 \\
\midrule \midrule
 \multirow{5}{*}{0.005} & \multirow{5}{*}{25.44} & \multirow{5}{*}{387.83}  & 20 & 4.61 & 0.17 & 0.00 & 97.80 \\
 &  &  & 30 & 4.25 & 0.18 & 43.33 & 97.80 \\
 &  &  & 40 & 3.54 & 0.17 & 66.67 & 97.81 \\
 &  &  & 50 & 4.13 & 0.15 & 80.0 & 97.80 \\
 &  &  & \texttt{NONE} & 2.17 & 0.17 & 86.67 & 97.84 \\ \midrule \midrule
 \multirow{4}{*}{0.003} & \multirow{4}{*}{15.93} & \multirow{4}{*}{248.10}  & 30 & 3.95 & 0.18 & 33.33 & 97.81 \\
 &  &  & 40 & 7.13 & 0.15 & 63.33 & 97.83 \\ 
  &  &  & 50 & 4.09 & 0.15 & 60.00 & 97.82 \\ 
 &  &  & \texttt{NONE} & 2.38 & 0.16 & 76.67 & 97.84 \\ \midrule \midrule
 \multirow{4}{*}{0.001} & \multirow{4}{*}{6.20} & \multirow{4}{*}{96.23}  & 30 & 4.82 & 0.14 & 3.33 & 97.85 \\
 &  &  & 40 & 4.34 & 0.14 & 10.00 & 97.82 \\
  &  &  & 50 & 3.80 & 0.14 & 16.67 & 97.86 \\
 &  &  & \texttt{NONE} & 3.06 & 0.16 & 23.33 & 97.85 \\ 
 \bottomrule
\end{tabular}
\label{table:results}
\end{table*}
